Multi-times Monte Carlo Rendering for Inter-reflection Reconstruction

Inverse rendering methods have achieved remarkable performance in reconstructing high-fidelity 3D objects with disentangled geometries, materials, and environmental light. However, they still face huge challenges in reflective surface reconstruction. Although recent methods model the light trace to learn specularity, the ignorance of indirect illumination makes it hard to handle inter-reflections among multiple smooth objects. In this work, we propose Ref-MC2 that introduces the multi-time Monte Carlo sampling which comprehensively computes the environmental illumination and meanwhile considers the reflective light from object surfaces. To address the computation challenge as the times of Monte Carlo sampling grow, we propose a specularity-adaptive sampling strategy, significantly reducing the computational complexity. Besides the computational resource, higher geometry accuracy is also required because geometric errors accumulate multiple times. Therefore, we further introduce a reflection-aware surface model to initialize the geometry and refine it during inverse rendering. We construct a challenging dataset containing scenes with multiple objects and inter-reflections. Experiments show that our method outperforms other inverse rendering methods on various object groups. We also show downstream applications, e.g., relighting and material editing, to illustrate the disentanglement ability of our method.

==> sections/intro.tex <==
% !TEX root = ../main.tex

\section{Introduction}
\label{sec:intro}

% 
% Texture editing is an important task in 3D modeling that involves manipulating the surface properties of 3D models to create a visually fantastic and appealing appearance according to the user's ideas. 
% With the increasing applications of 3D models in entertainment and e-shopping, 
% how to automatically generate and edit the texture of a 3D model without manual effort becomes an appealing task in the field of 3D vision.
% However, this task is challenging due to the complexity of 3D models and the special representation of the texture. 

To sufficiently handle the above applications, it would be desirable if a texture editing method can fulfill the following aspects: 
1) \textbf{Realism}: The generated textures should give rise to realistic and visually natural 2D images after rendering. It requires generative models to capture the complex patterns and structures present in the textures of the 3D model.
2) \textbf{Relighting}: The relighting ability allows adjusting the lighting conditions of the edited model to be consistent with the changes made to its texture.
3) \textbf{Efficiency}: Teexture editing should be efficient and scalable. This requires the use of fast and memory-efficient generative models that can generate high-quality textures in a short time.

Recent advances have demonstrated the effectiveness of generative models in synthesizing high-quality textures that are both visually pleasing and semantically meaningful. The use of generative adversarial networks (GANs)~\cite{DBLP:conf/cvpr/XianSARLFYH18,DBLP:conf/icml/BergmannJV17,DBLP:journals/tog/SunWSWWL22, chen2023hyperstyle3d} has shown promising results in producing textures with intricate patterns and complex structures. Other approaches, such as texture synthesis via direct optimization~\cite{DBLP:conf/iccv/EfrosL99,DBLP:journals/tog/FruhstuckAW19,DBLP:journals/tog/SendikC17a,DBLP:journals/tog/ZhouZBLC018} or neural style transfer~\cite{DBLP:journals/cgf/BerkitenHSMLR17,DBLP:journals/tog/HertzHGC20,DBLP:conf/aaai/WangZ0LZXL22,DBLP:conf/rt/MertensKCBD06}, have also been explored for their ability to generate textures with specific artistic styles. 
However, the capacity of these models is still unable to meet the need of real-world applications, which requires high-quality and diverse textures. 
Meanwhile, recent researches~\cite{chen2023fantasia3d,richardson2023texture,DBLP:journals/corr/abs-2211-07600,DBLP:journals/corr/abs-2211-10440, liu2023zero, kawar2022imagic, meng2021sdedit} on the diffusion models have emerged as a powerful new family of generative methods, which achieve impressive generation results in natural images and videos, inspiring us to introduce the awesome power into the task of 3D modeling.

However, directly applying the diffusion model to 3D objects is a non-trivial task due to the following reasons. 1) \textbf{The gap between the 3D representation and natural images.} Existing diffusion models are typically trained with natural images, making the pre-trained diffusion model lack prior knowledge in the 3D domain. Moreover, due to the complexity of the 3D model, it would be difficult to simultaneously edit shape, appearance, and shading, sometimes leading to conflicts in optimization goals. Therefore, directly editing the 3D representation may cause extreme semantic bias and destruction of inherent 3D topology. 2) \textbf{The learning misdirection of text description.} It is hard for text prompts to exactly describe the target images at the pixel level, leading to an ambiguous direction when taking the rendered images as the bridge. 

To solve these problems, we present an efficient model, dubbed ITEM3D, which can generate visually natural texture corresponding to the text prompt generated by users.
Instead of directly applying the diffusion model for texture editing in the 2D space, we adopt rendered images as the intermediary that bridges the text prompts and the appearance of 3D models. 
Apart from the appearance, the lighting and shading are also key components influencing the rendering results.
% However, the 3D object editing is much more than just manipulation the appearance along with the text prompts, as the shading is one of the key components influencing the rendering results.
Therefore, we represent the 3D model into a triangular mesh and a set of disentangled materials consisting of the texture and an environment map using nvdiffrec~\cite{munkberg2022extracting}, which achieves a balance for representing both appearance and shading.

To optimize a texture and an environment map with the diffusion model, a naive idea is to adopt the score distillation sampling (SDS) like 2D diffusion-based editing methods, which represents the absolute direction.
Unfortunately, the absolute direction often leads to noisy details and an inconsistent appearance, due to the ambiguous description of the text prompt for the target images.
Inspired by the recent improvement~\cite{DBLP:journals/corr/abs-2304-07090}, we replace the absolute editing direction led by the score distillation sampling with a relative editing direction determined by two predicted noises under the condition of the source text and the target text respectively, as illustrated in~\cref{fig:intro_1} (a). 
In this way, our model enables us to edit the texture in obedience to the text while bypassing the inconsistency problem by releasing the ambiguous description.
It is ideal that the intermediate states between the source and target text can give relatively accurate descriptions for arbitrary rendered images during the optimization, like the green straight lines in~\cref{fig:intro_1} (b).
However, the optimization in the texture domain actually shows an unexpected offset of the appearance in rendered images, leading to the deviation from the determined direction, like the red line in~\cref{fig:intro_1} (b).
To reduce the deviation caused by the texture projection, we gradually adjust the editing direction during the optimization, as green fold lines shown in~\cref{fig:intro_1} (b).
With the advent of the textural-inversion model, it can be easy to automatically correct the description as the change of the texture and its rendered images.

With the advent of the textural-inversion model, it can be easy to automatically correct the description as the change of the texture and its rendered images.


% In this paper, we present an efficient model, dubbed TexTexture, which can generate visually natural texture corresponding to the user's text prompt.
% We first reconstruct the 3D model into a triangular mesh and a set of spatially varying materials consisting of the texture and an environment map using nvdiffrec~\cite{}, which serves as the base for further text-guided editing.
% Given the explicit geometry and initial materials, our method further learns the texture and environment map to manipulate the appearance of rendered images under the condition of an input prompt. 
% The latent diffusion model~\cite{rombach2022high} takes the multi-view rendered images as the input and leverages the gradient of the difference between noises predicted by the U-Net~\cite{} as the optimization direction.
% The naive objective of optimization that maximizes score distillation sampling often leads to noisy details and inconsistent appearance, due to the ambiguous description of the text prompt for the target images.
% Inspired by the recent improvement~\cite{}, we replace the absolute editing direction led by the score distillation sampling with a relative editing direction along the difference between two predicted noises under the condition of source text and target text respectively, as illustrated in~\cref{fig:intro_1} (a). 
% In this way, our model enables to edit the texture in obedience to text while bypassing the inconsistency problem caused by the ambiguous description.

% However, the relative directional loss remains an important challenge that there exists \textbf{domain gap between natural images and texture images}.
% The relative direction severely depends on the accurate description of the source text prompts, while the optimization in texture domain shows unexpected offset of the appearance in rendered images.
% This offset leads to the deviation from the determined direction.
% To adapt our model across texture domain, we gradually adjust the editing direction during the optimization, as shown in~\cref{fig:intro_1} (b).
% With the advent of textural-inversion model, it can be easy to automatically correct the description as the change of texture and rendered images.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figs/direction.png}
   \caption{\textbf{Motivation}. (a) Previous methods~\cite{DBLP:journals/corr/abs-2209-14988, chen2023fantasia3d} with SDS Loss to directly guide the optimization leads to ambiguous details due to the bias between texts and images (red line), while our method introduces the relative direction between source and target texts to the optimization process, eliminating the bias and improving the rendering results (green line). (b) The optimization in the texture domain gives rise to the deviation of the target direction (red line), thus we gradually adjust the direction to fine-tune the optimization (fold green line).}
   \label{fig:intro_1}
\end{figure}

Thanks to the proposed solutions, our method overcomes the challenges of domain gap and learning misdirection, fulfilling all three requirements of texture editing.
In summary, our contributions are:
\begin{itemize}[leftmargin=2.5em]
\setlength\itemsep{0em}
\item We design an efficient optimization pipeline to edit the texture and environment map obedient to the text prompt, directly empowering the downstream application in the industrial pipeline.
\item We introduce the relative direction to the 3D texture optimization, releasing the problem of noisy details and inconsistent appearance caused by the semantic ambiguity between the texts and images.
\item We propose to gradually adjust the relative direction guided by the source and target texts which addresses the unexpected deviation from the determined direction caused by the texture.
\end{itemize}


==> sections/methods.tex <==
%------------------------------------------------------------------------
\section{Method}
\subsection{Overview}
Given a set of multi-view images $\mathcal{I}=\{I_{1}, ..., I_{n}\}$, we aim to reconstruct the 3D model with both geometry and texture, and then edit the texture under the guidance of text prompts.
To this end, we design a zero-shot differentiable framework that optimizes the disentangled materials of the object, \ie texture map and environment map.
%solving the challenge of 3D inconsistency caused by the inconsistent 2D training images.
We first leverage a differentiable rendering model $\mathcal{R}$ to represent the 3D model as an accurate shape and surface materials with texture and environment map \cref{sec:Representation}).
For further editing of appearance, we utilize the diffusion model to guide the direction of the texture optimization given the target text prompt.
To solve the problem of ambiguous and noisy details, we introduce the relative direction of source text and target text into the optimization (\cref{sec:Relative direction}). 
Moreover, we gradually adjust relative direction to address the challenges of deviation caused by the unbalanced optimization in the texture domain (\cref{sec:Adjustment}).
The overview of our method is demonstrated in~\cref{fig:method_1}.

\subsection{3D Model Representation}
\label{sec:Representation}
% To accomplish editing the appearance of the 3D model via text prompt, we utilize a triangular mesh and a set of spatially varying materials as the 3D representation. 
% By disentangling the 3D model into the geometry part and the appearance part, we edit the texture directly while keeping the geometry invariant.
To accomplish editing the appearance of the 3D model via text prompt, we disentangle the 3D model into a triangular mesh and a set of spatially varying materials. The disentanglement thus allows us to edit the texture directly while keeping the geometry invariant.
The material model we employed combines a diffuse term, a specular term and a normal term.
A four-channel texture is provided for the diffuse parameters $k_d$, where the optional fourth channel $\alpha$ represents the transparency.
Meanwhile, the specular term is described by a roughness factor $r$, a metalness factor $m$ and a sheen factor $o$ that is unused in our model.
% The specular highlight color $k_s$ can then be computed by $k_s = (1 - m) \cdot 0.04 + m \cdot k_d$. 
These values $(o,r,m)$ are stored in another texture map $k_{orm}$.
The normal term in our representation is a tangent space normal map $n$, which is utilized to capture the high-frequency details of the appearance.
In order to handle texturing effectively during optimization, we utilize volumetric texturing and access our texture by the world space position $x$.
% This specific approach guarantees that the mapping adjusts seamlessly while keeping the topology unchanged.
% Furthermore, 
We tackle the challenge of the impractical cubic growth in memory usage of volumetric textures for our target resolution by leveraging a multi-layer perceptron (MLP) to encode the material parameters into a compact representation.
Specifically, given a world space position $x$, we compute the base color, $k_d$, the specular parameters, $k_{orm}$ and a tangent space normal perturbation $n$, the mapping is thus formulated as $x \rightarrow (k_d, k_{orm}, n)$.
With the introduction of this mapping, for a fixed topology, the textures are initialized by sampling the MLP on the mesh surface and then optimized efficiently. Following the rendering equation of the image-based lighting model, we compute the radiance $L$ in direction $\omega_o$ by:
\begin{equation}
L\left(\omega_o\right)=\int_{\Omega} L_i\left(\omega_i\right) f\left(\omega_i, \omega_o\right)\left(\omega_i \cdot \mathbf{n}\right)d\omega_i ,
\label{eq:render}
\end{equation}
where $L_i$ is the incident radiance from direction $\omega_i$ , the $f$ is the BSDF and $n$ is the intersection normal of the corresponding integral domain $\Omega$. Specifically, we adopt the Cook-Torrance microfacet specular shading model as the BSDF in our rendering equation:
\begin{equation}
f\left(\omega_i, \omega_o\right)=\frac{D\ G\ F}{4\left(\omega_o \cdot \mathbf{n}\right)\left(\omega_i \cdot \mathbf{n}\right)}.
\label{eq:bsdf}
\end{equation}
The term $D$ here represents the GGX~\cite{DBLP:conf/rt/WalterMLT07} normal distribution while the term $G$ is the geometric attenuation and $F$ is the Fresnel
term respectively. Furthermore, we employ the split-sum approximation for its efficiency and the rendering equation~\cref{eq:render} can be formulated as:
\begin{equation}
L\left(\omega_o\right) \approx \int_{\Omega} f\left(\omega_i, \omega_o\right)\left(\omega_i \cdot \mathbf{n}\right) d \omega_i \int_{\Omega} L_i\left(\omega_i\right) D\left(\omega_i, \omega_o\right)\left(\omega_i \cdot \mathbf{n}\right) d \omega_i.
\end{equation}
The first term of this product only relies on the parameters $\left(\omega_i \cdot \mathbf{n}\right)$ and the roughness $r$ of the BSDF, which are precomputed and stored in a 2D lookup texture. Meanwhile, the second term is the integral of the radiance with the specular normal distribution function $D$ expressed in~\cref{eq:bsdf}, which is also precomputed and stored by a filtered cubemap. Owing to the precomputation and lookup mechanism, the rendering process is then accelerated. In order to learn the environment lighting from 2D image observations, we employ a differentiable shading model to represent this split-sum approximation. The cube map in our case can be represented as trainable parameters, which are initialized as the preintegrated lighting. 


\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figs/pipeline.png}
   \caption{\textbf{Pipeline} of texture editing. We render the 3D model with mesh, texture, and environment map into 2D images which are then added with noise $\epsilon$. We then use the source text and the target text as the conditions to denoise via two U-Nets. The difference between the two predicted noises serve as the relative direction to guide the optimization of the materials of the 3D model, \ie texture and environment map.}
   \label{fig:method_1}
\end{figure}

\subsection{Relative Direction Based Optimization}
\label{sec:Relative direction}
Our goal is to enable users to edit the appearance of 3D models using natural language descriptions. 
To accomplish this, the directional idea is to utilize the diffusion model that has been pre-trained in 2D images as knowledge prior to guide the editing of texture.
% In our model, we utilize the Physically Based Rendering (PBR) material model as the 3D representation which disentangles the 3D model into three components, i.e., the texture map $K_{d}$, the environment lighting $K_{l}$ and the normal map $K_{n}$.
% Keeping the normal map constant, we opt to jointly optimize the texture map $K_{d}$ and the environment light $K_{m}$ with the objective of the Distillation Sampling Loss.
Naively, we could use Score Distillation Sampling (SDS) loss,
\begin{equation}
    \nabla_{\theta}\mathcal{L}_{\mathrm{SDS}}(\phi, \mathbf{x}=\mathcal{R}(\theta))=\mathbb{E}_{t,\epsilon}\left[w(t)\left(\epsilon_{\phi}^{\omega}(\mathbf{z}_t;y,t)-\epsilon\right)\frac{\partial\mathbf{x}}{\partial\theta}\right],
\end{equation}

where $\mathbf{x}$ is the rendered images, $t$ is the sampled time step, $z_t$ is the $t$ time step latent, $w(t)$ is the weighting function that equals $\partial\mathbf{z}_t / \partial\mathbf{x}$, $y$ is the text condition, $\epsilon_{\phi}^{\omega}(\mathbf{z}_t;y,t)$ is the predicted noise through classifier-free guidance, and $\epsilon \in N (0, I)$ is the noise added to the rendered images.
The gradient of SDS loss gives an editing direction for our texture optimization, determined by the text prompt $y$.
However, the SDS loss may cause the destruction of original image content with noisy details, because the text prior typically cannot faithfully reflect the information of the image.
% These shortcomings make this loss unsuitable for train
It is known that the entropy of an RGB image is significantly larger than that of a text prompt.
As a consequence, the misdescription inevitably arises when taking the text prompt as the prior to restore the high-quality image from the same-scale noise.
Therefore, even for a text prompt $y_{0}$ describing the original images, there exists a deviation related to the optimized texture $\theta$ between the added noise $\epsilon$ and the predicted noise $\epsilon_{\phi}^{\omega}\left(\mathbf{z}_{t};y_{0},t\right)$, which can be simply expressed as, 
\begin{equation}
    D_{\mathrm{bias}}(\theta, ... ) \propto ||\epsilon_{\phi}^{\omega}\left(\mathbf{z}_{t};y_{0},t\right)-\epsilon||.
\end{equation}

Thus, the gradient leads to a bias term from the original input image, which can be expressed as, 
\begin{equation}
    \Vec{n}_{\rm bias} = \frac{\partial D_{\mathrm{bias}}(\theta, ...)}{\partial\theta}  = \left(\epsilon_{\phi}^{\omega}\left(\mathbf{z}_{t};y_{0},t\right)-\epsilon\right)\frac{\partial\mathbf{x}}{\partial\theta}.
\end{equation}
Moreover, for an arbitrary text prompt $y_{\rm tgt}$ describing the target editing texture, it could be considered that there exists a term of expected editing direction and a term of bias discussed above, 

\begin{equation}
    \left(\epsilon_{\phi}^{\omega}\left(\mathbf{z}_{t};y_{\rm tgt},t\right)-\epsilon\right)\frac{\partial\mathbf{x}}{\partial\theta} = \Vec{n}_{\rm tgt} + \Vec{n}_{\rm bias}.
\end{equation}

As a result, the $\Vec{n}_{\rm bias}$ gives rise to the misdirection for the optimization procedure.

To address these issues, it is ideal to find the accurate editing direction $\Vec{n}_{\rm tgt}$, while the term of $\Vec{n}_{\rm bias}$ is hard to estimate due to the diverse input images.
To mitigate the gap, it is natural to take the text guidance as a relative direction rather than an absolute direction, enabling us to eliminate the term of $\Vec{n}_{\rm bias}$.
The absolute direction of the source $\Vec{n}_{\rm src}$ and the target $\Vec{n}_{\rm tgt}$ can be expressed as,
\begin{equation}
    \Vec{n}_{\rm src} = \left(\epsilon_{\phi}^{\omega}\left(\mathbf{z}_{t};y_{0},t\right)-\epsilon\right)\frac{\partial\mathbf{x}}{\partial\theta} - \Vec{n}_{\rm bias} ,
\end{equation}

\begin{equation}
    \Vec{n}_{\rm tgt} = \left(\epsilon_{\phi}^{\omega}\left(\mathbf{z}_{t};y_{\rm tgt},t\right)-\epsilon\right)\frac{\partial\mathbf{x}}{\partial\theta} - \Vec{n}_{\rm bias},
\end{equation}

where $\Vec{n}_{\rm src}$ is actually the $\Vec{0}$ giving no extra information to the input images.
Inspired by the CLIP-directional loss improved by the StyleGAN-Nada~\cite{DBLP:journals/tog/GalPMBCC22} and the denoising loss proposed by the recent work~\cite{DBLP:journals/corr/abs-2209-14988}, we utilize the difference between the source $\Vec{n}_{\rm src}$ and the target $\Vec{n}_{\rm tgt}$ as the relative direction of the target, which can be presented as, 

\begin{equation}
    \Vec{n}_{\rm tgt}  = \Vec{n}_{\rm tgt} - \Vec{n}_{\rm src} = \left(\epsilon_{\phi}^{\omega}\left(\mathbf{z}_{t},y_{\rm tgt},t\right)-\epsilon_{\phi}^{\omega}\left(\mathbf{x},y_{0},t\right)\right)\frac{\partial\mathbf{x}}{\partial\theta}.
\end{equation}

Therefore, the final gradient utilized for optimizing the texture can be presented as,
\begin{equation}
    \nabla_{\theta}\mathcal{L}_{\mathrm{RDL}}(\phi, \mathbf{x}=\mathcal{R}(\theta))=\mathbb{E}_{t,\epsilon}\left[w(t)\left(\epsilon_{\phi}^{\omega}(\mathbf{z}_t;y_{\rm tgt},t)-\epsilon_{\phi}^{\omega}(\mathbf{z}_t;y_{0},t)\right)\frac{\partial\mathbf{x}}{\partial\theta}\right],
\end{equation}


\subsection{Direction Adjustment}
\label{sec:Adjustment}
Different from the gradual transition in the nature image domain, the optimization of the texture domain unfortunately shows an unexpected offset of the appearance in rendered images, due to the complex projection in differentiable rendering.
The inherent reason is that the complexity of rendering leads to unbalanced optimization for the texture, with some parts under-tuning and other parts over-tuning.
This appearance offset can be seen in some parts of the rendered image, leading to the inconsistency between the source text and the rendered images in the median period of the optimization procedure.
It is known that a source image with an inconsistent text description means an optimization misdirection which leads to an unknown change in the editing results.
Similar to the known problem, if a rendered image during the median optimization hops out the direction between the source text and the target text, it can be considered as the inconsistent description for the source image when we take the current median point as a relative beginning point.
The original editing direction is give by, 
\begin{equation}
    \Vec{n}_{\rm ori} = \Vec{n}_{\rm tgt} - \Vec{n}_{\rm src}.
\end{equation}
If the optimization continues along the original direction, a more severe deviation can be attached to the optimization procedure.

To avoid the misdirection caused by the texture domain, we propose to adjust the editing direction, specifically the source text prompt, during our optimization process of the texture map. The adjusted direction $\mathrm{\Delta}\hat{T}_{i}$ can be represented as, 
\begin{equation}
    \mathrm{\Delta}\hat{T}_{i} = \Vec{\hat{n}}_{i} - \Vec{\hat{n}}_{i-1} = \mathcal{B}(I_{i}) - \mathcal{B}(I_{i-1}),
\end{equation}
where $i$ is the optimization iteration and $\mathcal{B}\left( \bm{\cdot} \right)$ expresses the inverse text generated by a pre-trained language-image model BLIP-v2~\cite{li2023blip}. 

As shown in the~\cref{fig:intro_1} (b), the direction is continually adjusted during the optimization so that the new global direction $\Vec{n}_{i}$ can be written as, 
\begin{equation}
    \Vec{n}_{i} = \Vec{n}_{\rm ori} + \sum_{j \leq i}{ \mathrm{\Delta}\hat{T}_{j}}.
\end{equation}
By adjusting the optimization direction step by step, 
we achieve more delicate and controllable editing, which can be seen in~\cref{sec:dir_adjust}.

